Data-driven model predictive control of battery storage units

In many state-of-the-art control approaches for power systems with storage units, an explicit model of the storage dynamics is required. With growing numbers of storage units, identifying these dynamics can be cumbersome. This paper employs recent data-driven control approaches that do not require an explicit identification step. Instead, they use measured input/output data in control formulations. In detail, we propose an economic data-driven model predictive control (MPC) scheme to operate a small power system with input-nonlinear battery dynamics. First, a linear data-driven MPC approach that uses a slack variable to account for plant-model-mismatch is proposed. In a second step, an input-nonlinear data-driven MPC scheme is deduced. Comparisons with a reference indicate that the linear data-driven MPC approximates the nonlinear plant in an acceptable manner. Even better results, however, can be obtained with the input-nonlinear data-driven MPC scheme which provides increased prediction accuracy.

==> figures/newNodeCommands.tex <==
% !TeX encoding = UTF-8
% !TeX spellcheck = en_GB
% !TEX TS-program = pdflatex
% !TEX root = ../paper.tex

\newcommand{\GraphLine}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
	\path[line join=miter,line cap=round,miter
	limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
	rectangle (24,1);
	\path[draw, line width=\lnwidth] (7, 0.5) -- (17, 0.5); 
	\end{tikzpicture}}

\newcommand{\GraphLineFlip}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex, rotate=90]
	\path[line join=miter,line cap=round,miter
	limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
	rectangle (24,1);
	\path[draw, line width=\lnwidth] (7, 0.5) -- (17, 0.5); 
	\end{tikzpicture}}

\newcommand{\GraphTransformer}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
	\path[line join=miter,line cap=round,miter
	limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
	rectangle (24,24);
	\path[draw=none, fill=white, line width=\lnwidth] (12, 15) circle (6);
	\path[draw, fill=white, line width=\lnwidth] (12, 9) circle (6);
	\path[draw=, line width=\lnwidth] (12, 15) circle (6);
	\end{tikzpicture}}

\newcommand{\GraphTransformerFlip}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex, rotate=90]
	\path[line join=miter,line cap=round,miter
	limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
	rectangle (24,24);
	\path[draw=none, fill=white, line width=\lnwidth] (12, 15) circle (6);
	\path[draw, fill=white, line width=\lnwidth] (12, 9) circle (6);
	\path[draw=, line width=\lnwidth] (12, 15) circle (6);
	\end{tikzpicture}}

\newcommand{\GraphInverter}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
	\path[line join=miter, line cap=round, miter limit=4.00, line width=\lnwidth,
			rounded corners=0.0000cm] (0,0) rectangle (24,24);
	\path[draw, line join=miter, line cap=butt, miter limit=4.00, line width=\lnwidth] (22, 2) -- (2, 22);
	\draw [line width=\lnwidth] plot [smooth, tension=1] coordinates { (21, 19) (18, 16) (15, 19) (12, 16)};
	\draw [line width=\lnwidth]
		(4, 5.25) -- (11, 5.25)
		(4, 7.75) -- (11, 7.75);
	\end{tikzpicture}}

\newcommand{\GraphInverterFlip}{\begin{tikzpicture}[scale = \scaleSymbols*20/24, >=latex]
	\path[line join=miter, line cap=round, miter limit=4.00, line width=\lnwidth,
	rounded corners=0.0000cm] (0,0) rectangle (24,24);
	\path[draw, line join=miter, line cap=butt, miter limit=4.00, line width=\lnwidth] (22, 2) -- (2, 22);
	\draw [line width=\lnwidth] plot [smooth, tension=1] coordinates { (21, 19) (18, 16) (15, 19) (12, 16)};
	\draw [line width=\lnwidth]
	(4, 5.25) -- (11, 5.25)
	(4, 7.75) -- (11, 7.75);
	\end{tikzpicture}}

\newcommand{\tower}{\begin{tikzpicture}[scale = \scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
         limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] 
				(0,0)
       rectangle (24,24);
   \draw (-1,0) arc (180:360:1cm and 0.5cm);
    \draw (-1,0) arc (180:0:1cm and 0.5cm);
    \draw (-2,-3) arc (180:360:2cm and 1cm);
    %\draw[dashed] (-2,-3) arc (180:10:2cm and 1cm);
    \draw(-2,-3)  -- (-1,0);
    \draw(2,-3)   -- (1,0);
    \shade[left color=blue!5!white,right color=blue!60!white,opacity=0.3] (-1,0) arc (180:360:1cm and 0.5cm) -- (2,-3) arc (360:180:2cm and 1cm) -- cycle;
    \shade[left color=blue!5!white,right color=blue!60!white,opacity=0.3] (0,0) circle (1cm and 0.5cm);
\end{tikzpicture}
}

\newcommand{\GraphTristateFC}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
        rectangle (24,24);
      %\path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (0,12) -- (9,12) -- (15,6);
      \path[draw,fill,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth,color=black!50!white] (18,4) rectangle (15,20);
      \path[draw,fill,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth,color=black!80!white] (13,4) rectangle (11,20);
      \path[draw,fill,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth,color=black!50!white] (9,4) rectangle (6,20);
\end{tikzpicture}}

\newcommand{\GraphTristateTF}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
        rectangle (24,24);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (0,12) -- (4,12);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (20,12) -- (24,12);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (15,12) circle (5);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (9,12) circle (5);
\end{tikzpicture}}

\newcommand{\GraphTristatePCC}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
        rectangle (24,24);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (0,12) -- (9,12) -- (15,6);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (15,12) -- (24,12);
\end{tikzpicture}}

\newcommand{\GraphTristateR}{
%	\renewcommand{\linewidthR}m}
\begin{tikzpicture}[scale = \scaleSymbols, >=latex, color=black]
        \path[] (315.0000,52.3622-1) rectangle (335.0000,72.3622-1);
        \path[draw,fill,line join=round,line cap=round,miter limit=4.00,line
          width=\lnwidth] (324.0306,59.8874) .. controls (321.9302,58.2551) and
          (319.7014,56.9114) .. (317.2333,55.6929) .. controls (319.8093,57.9660) and
          (324.1469,60.6035) .. (324.0306,59.8874) -- cycle;
        \path[draw,fill,line join=round,line cap=round,miter limit=4.00,line
          width=\lnwidth] (325.5865,60.4167) .. controls (328.0392,59.6017) and
          (330.4240,58.6404) .. (332.7667,57.0558) .. controls (329.8032,57.9971) and
          (326.8503,59.6115) .. (325.5865,60.4167) -- cycle;
        \path[draw,fill,line join=round,line cap=round,miter limit=4.00,line
          width=\lnwidth] (324.8607,61.1176) .. controls (324.6795,63.5961) and
          (324.6662,66.1651) .. (325.3315,69.0315) .. controls (325.5549,66.1044) and
          (325.1090,62.6873) .. (324.8607,61.1176) -- cycle;
        \path[cm={{0.20207,0.0904,-0.09626,0.21517,(296.36236,26.26027)}},draw,fill,line
          join=round,line cap=round,miter limit=4.00,line width=\lnwidth]
          (186.0000,84.3622) .. controls (186.0000,86.6957) and (183.5376,88.5874) ..
          (180.5000,88.5874) .. controls (177.4624,88.5874) and (175.0000,86.6957) ..
          (175.0000,84.3622) .. controls (175.0000,82.0287) and (177.4624,80.1370) ..
          (180.5000,80.1370) .. controls (183.5376,80.1370) and (186.0000,82.0287) ..
          (186.0000,84.3622) -- cycle;
\end{tikzpicture}
}

%===================

\newcommand{\GraphTristateS}{
\begin{tikzpicture}[scale = -\scaleSymbols, >=latex, color=black]
        \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (265.0000,52.3622)
          rectangle (285.0000,72.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (269.0000,61.3622) -- (281.0000,61.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (275.0000,55.3622) -- (275.0000,61.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (272.0000,63.3622) -- (278.0000,63.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (275.0000,63.3622) -- (275.0000,69.3622);
\end{tikzpicture}
}


\newcommand{\GraphTristateL}{
\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex, color=black]
      \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (231.3607,117.8948)
        rectangle (255.3607,141.8948);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line
        width=\lnwidth, <-] (243.3607,137.3622) -- (243.3607,124.4274);
\end{tikzpicture}
}

% %===================

\newcommand{\GraphTristateT}{
\begin{tikzpicture}[scale = -\scaleSymbols, >=latex, color=black]
        \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (495.0000,52.3622-.5)
          rectangle (515.0000,72.3622-.5);
        \path[cm={{0.38462,0.0,0.0,0.83333,(380.9615,-59.27301)}},draw, line
          join=round,line cap=round,miter limit=4.00,line width=\lnwidth, color = black]
          (342.0000,145.3622) .. controls (342.0000,150.3328) and (333.2695,154.3622) ..
          (322.5000,154.3622) .. controls (311.7305,154.3622) and (303.0000,150.3328) ..
          (303.0000,145.3622) .. controls (303.0000,140.3916) and (311.7305,136.3622) ..
          (322.5000,136.3622) .. controls (333.2695,136.3622) and (342.0000,140.3916) ..
          (342.0000,145.3622) -- cycle;
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth, color = black]
          (505.0000,54.3622) -- (505.0000,69.3622);
\end{tikzpicture}
}


% %===================

\newcommand{\GraphTristateP}{
\begin{tikzpicture}[scale = -\scaleSymbols, >=latex, color=black]
        \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (495.0000,52.3622)
          rectangle node {N} (515.0000,72.3622) ;
\end{tikzpicture}
}

% %===================

\newcommand{\GraphTristatePV}{
\begin{tikzpicture}[scale =  -\scaleSymbols, >=latex, color=black]
%=== PV ===
  \begin{scope}[cm={{1.33333,0.0,0.0,1.33333,(-219.66665,-77.45405)}}]
    \path[line join=miter,line cap=round,miter
      limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (371.0000,157.3622)
      rectangle (386.0000,172.3622);
    \begin{scope}[cm={{0.75,0.0,0.0,0.75,(108.84792,54.02778)}}]
      \path[cm={{0.45455,0.21485,-0.21652,0.51139,(295.25671,66.03768)}},draw,fill,line
        join=round,line cap=round,miter limit=4.00,line width=\lnwidth]
        (186.0000,84.3622) .. controls (186.0000,86.6957) and (183.5376,88.5874) ..
        (180.5000,88.5874) .. controls (177.4624,88.5874) and (175.0000,86.6957) ..
        (175.0000,84.3622) .. controls (175.0000,82.0287) and (177.4624,80.1370) ..
        (180.5000,80.1370) .. controls (183.5376,80.1370) and (186.0000,82.0287) ..
        (186.0000,84.3622) -- cycle;
      \begin{scope}[shift={(-0.46388,0.41703)}]
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (362.2097,144.9631) -- (368.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,151.3622) -- (356.4103,149.0251);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (363.3146,147.2675) -- (368.0000,147.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,143.3622) -- (356.1804,145.6575);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (368.0000,155.3622) -- (362.5254,149.6350);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (358.2954,144.1423) -- (356.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (360.0000,155.3622) -- (359.9369,151.0555);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,155.3622) -- (357.0000,150.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,147.3622) -- (356.2119,147.4569);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,139.3622) -- (357.1274,144.7105);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (359.8422,144.3002) -- (360.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (361.3258,144.2370) -- (364.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (356.0000,155.3622) -- (358.2954,150.8977);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (362.6832,145.9732) -- (368.0000,142.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (363.2514,148.3092) -- (368.0000,149.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (364.6693,154.2802) -- (361.4307,150.5189);
      \end{scope}
    \end{scope}
  \end{scope}
\end{tikzpicture}
} 
